ACE : Off-Policy Actor-Critic with Causality-Aware Entropy Regularization

The varying significance of distinct primitive behaviors during the policy learning process has been overlooked by prior model-free RL algorithms. Leveraging this insight, we explore the causal relationship between different action dimensions and rewards to evaluate the significance of various primitive behaviors during training. We introduce a causality-aware entropy term that effectively identifies and prioritizes actions with high potential impacts for efficient exploration. Furthermore, to prevent excessive focus on specific primitive behaviors, we analyze the gradient dormancy phenomenon and introduce a dormancy-guided reset mechanism to further enhance the efficacy of our method. Our proposed algorithm, ACE: Off-policy Actor-critic with Causality-aware Entropy regularization, demonstrates a substantial performance advantage across 29 diverse continuous control tasks spanning 7 domains compared to model-free RL baselines, which underscores the effectiveness, versatility, and efficient sample efficiency of our approach. Benchmark results and videos are available at https://ace-rl.github.io/.

==> algorithms/cac.tex <==
\begin{algorithm}
\caption{off-policy Actor-critic with Causality-aware Entropy~(\ours)}
\begin{algorithmic}
    \STATE \textbf{initialize:} Q network $Q_{\phi}$, policy network $\pi_\theta$, replay buffer $\mathcal{D}$; local buffer $\mathcal{D}_c$ with size $N_c$, causal weight matrix $\rmB_{\rva\rightarrow r\vert \rvs}$, perturb factor $f$; 
    
    \FOR{each environment step $t$}
        \STATE Collect data with $\pi_\theta$ from real environment
        \STATE Add to replay buffer $\mathcal{D}$ and local buffer   $\mathcal{D}_c$
    \ENDFOR
    \STATE \textcolor{myblue}{// Causal discovery}
    \IF{every $I$ environment step}
        \STATE Sample all $N_c$ transitions from local buffer $\mathcal{D}_c$
        \STATE Update causal weight matrix \textcolor{red}{$\rmB_{\rva\rightarrow r\vert \rvs}$}
    \ENDIF
    \FOR{each gradient step}
        \STATE Sample $N$ transitions $(\rvs, \rva,r,\rvs')$ from $\mathcal{D}$
        \STATE \textcolor{myblue}{// Policy evaluation}
        \STATE Compute causal policy-reward entropy \textcolor{red}{$\mathcal{H}_c(\pi(\cdot\vert \rvs))$} 
        \STATE Calculate the target $Q$ value
        \STATE Update $Q_{\phi}$ by $\min_\phi\left(\mathcal{T}_cQ_{\phi}-Q_{\phi}\right)^2$
        \STATE \textcolor{myblue}{// Policy optimization}
        \STATE Update $\pi_\theta$ by $\max_{\theta} Q_\phi(s,a)$
    \ENDFOR
    \STATE \textcolor{myblue}{// Gradient-guided Perturbation}
    \IF{every $P$ environment step}
        \STATE Calculate the gradient dormant ratio $\beta_{\gamma}$
        \STATE Perturb $Q_{\phi}$ and $\pi_\theta$ with factor $f(\beta_{\gamma})$
    \ENDIF
\end{algorithmic}
\label{purealg:cac}
\end{algorithm}
